Dynamical analysis of quantum matter bounces with dark sector mimickers

We study the effects of the inclusion of fluids In bounce scenarios driven by an exponential potential scalar field. Most solutions exhibit well known tracking behavior between the fluids and the scalar field. This tracking behavior can model transitions between different phases of cosmic evolution. We will focus on an interesting bouncing model with a dust matter fluid, where the scalar field can drive an early dark energy expanding period with a radiation-like dominated phase just after it, and then tracks the dust matter fluid with energy density compatible with the dark matter energy density. The model is dust dominated in the far past of the contracting phase, and has stiff matter behavior when approaching the singularity, allowing well known quantum bounce transitions to the expanding era. Hence, it is a quantum matter bounce scenario with an inflationary phase together with a smooth transition through a radiation era to matter domination with a possible scalar field dark matter candidate.

==> sections/acknowledgements.tex <==
\section*{Acknowledgements} \label{sec:acknowledgements}
